JSMoCo: Joint Coil Sensitivity and Motion Correction in Parallel MRI with a Self-Calibrating Score-Based Diffusion Model

Magnetic Resonance Imaging (MRI) stands as a powerful modality in clinical diagnosis. However, it is known that MRI faces challenges such as long acquisition time and vulnerability to motion-induced artifacts. Despite the success of many existing motion correction algorithms, there has been limited research focused on correcting motion artifacts on the estimated coil sensitivity maps for fast MRI reconstruction. Existing methods might suffer from severe performance degradation due to error propagation resulting from the inaccurate coil sensitivity maps estimation. In this work, we propose to jointly estimate the motion parameters and coil sensitivity maps for under-sampled MRI reconstruction, referred to as JSMoCo. However, joint estimation of motion parameters and coil sensitivities results in a highly ill-posed inverse problem due to an increased number of unknowns. To address this, we introduce score-based diffusion models as powerful priors and leverage the MRI physical principles to efficiently constrain the solution space for this optimization problem. Specifically, we parameterize the rigid motion as three trainable variables and model coil sensitivity maps as polynomial functions. Leveraging the physical knowledge, we then employ Gibbs sampler for joint estimation, ensuring system consistency between sensitivity maps and desired images, avoiding error propagation from pre-estimated sensitivity maps to the reconstructed images. We conduct comprehensive experiments to evaluate the performance of JSMoCo on the fastMRI dataset. The results show that our method is capable of reconstructing high-quality MRI images from sparsely-sampled k-space data, even affected by motion. It achieves this by accurately estimating both motion parameters and coil sensitivities, effectively mitigating motion-related challenges during MRI reconstruction.

==> Table/main_result_table.tex <==
% \usepackage{multirow}


\begin{table*}
\centering
\caption{hhh}
\label{table_com}
\begin{tabular}{ccccccccc} 
\toprule
\textbf{Accelerate} & \multicolumn{2}{c}{\textbf{Motion Setting}} & \multicolumn{6}{c}{\textbf{Method}}\\ 
\cmidrule{2-3}
\textbf{Rate} & \textbf{Rotate}             & \textbf{Translate}      & \textbf{ZF} & \textbf{L1-Wavelet} & \textbf{E2E-VN} & \textbf{NAMER}              & \textbf{Score-MoCo}           & \textbf{Ours}                  \\ 

\midrule
\multirow{4}{*}{$\times$2} &\multirow{2}{*}{$\pm$ 2$^\circ$} & $\pm$ 3 pixels             &    &            &        &                      &                      &                       33.67/0.9397 
 \\
               &    & $\pm$ 4 pixels             &    &            &        &                      &                      &          33.38/0.9378 
             \\ 
\cmidrule{2-9}
& \multirow{2}{*}{$\pm$ 3$^\circ$} & $\pm$ 3 pixels             &    &            &        &                      &                      &                        33.94/0.9391\\
              &     & $\pm$ 4 pixels             &    &            &        &                      &                      &      34.65/0.9419                  \\
\midrule
\multirow{4}{*}{$\times$4} &\multirow{2}{*}{$\pm$ 2$^\circ$} & $\pm$ 3 pixels             &    &            &        &                      &                      &                  

    33.13/0.9270\\
               &    & $\pm$ 4 pixels             &    &            &        &                      &                      &                        32.49/0.9272\\ 
\cmidrule{2-9}
& \multirow{2}{*}{$\pm$ 3$^\circ$} & $\pm$ 3 pixels             &    &            &        &                      &                      &                        32.47/0.9258\\
              &     & $\pm$ 4 pixels             &    &            &        &                      &                      &                        32.29/0.9233\\
\midrule
\multirow{4}{*}{$\times$4.8} &\multirow{2}{*}{$\pm$ 2$^\circ$} & $\pm$ 3 pixels             &    &            &        &                      &                      &                

    31.95/0.9195\\
               &    & $\pm$ 4 pixels             &    &            &        &                      &                      &                        30.57/0.9136\\ 
\cmidrule{2-9}
& \multirow{2}{*}{$\pm$ 3$^\circ$} & $\pm$ 3 pixels             &    &            &        &                      &                      &                        31.41/0.9180\\
              &     & $\pm$ 4 pixels             &    &            &        &                      &                      &                       31.75/0.9218 \\
\bottomrule
\end{tabular}
\end{table*}
